Automated Long Answer Grading with RiceChem Dataset

We introduce a new area of study in the field of educational Natural Language Processing: Automated Long Answer Grading (ALAG). Distinguishing itself from Automated Short Answer Grading (ASAG) and Automated Essay Grading (AEG), ALAG presents unique challenges due to the complexity and multifaceted nature of fact-based long answers. To study ALAG, we introduce RiceChem, a dataset derived from a college chemistry course, featuring real student responses to long-answer questions with an average word count notably higher than typical ASAG datasets. We propose a novel approach to ALAG by formulating it as a rubric entailment problem, employing natural language inference models to verify whether each criterion, represented by a rubric item, is addressed in the student's response. This formulation enables the effective use of MNLI for transfer learning, significantly improving the performance of models on the RiceChem dataset. We demonstrate the importance of rubric-based formulation in ALAG, showcasing its superiority over traditional score-based approaches in capturing the nuances of student responses. We also investigate the performance of models in cold start scenarios, providing valuable insights into the practical deployment considerations in educational settings. Lastly, we benchmark state-of-the-art open-sourced Large Language Models (LLMs) on RiceChem and compare their results to GPT models, highlighting the increased complexity of ALAG compared to ASAG. Despite leveraging the benefits of a rubric-based approach and transfer learning from MNLI, the lower performance of LLMs on RiceChem underscores the significant difficulty posed by the ALAG task. With this work, we offer a fresh perspective on grading long, fact-based answers and introduce a new dataset to stimulate further research in this important area. Code: \url{https://github.com/luffycodes/Automated-Long-Answer-Grading}.

==> figures/comparison.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/comparison_accuracy.pdf}
    %\caption{Caption for Figure 1}
    \label{fig:comparison_acc}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/comparison_f1.pdf}
    %\caption{Caption for Figure 2}
    \label{fig:comparison_f2}
  \end{subfigure}
  \captionsetup{skip=0pt}
  \caption{Comparisons between the traditional ASAG approach and \model on the \dataset dataset.
  \model offers an average increase of $9.2\%$ in accuracy and an average increase of $15.4\%$ in F1 score, proving that breaking down grading into smaller rubric items helps models focus on smaller parts of the task instead of doing the entire task altogether. The improvement is evident across all models regardless of their number of parameters.}
  \label{fig:comparison}
\end{figure*}

==> sections/ethics.tex <==
Our study involves collecting a dataset of college-level chemistry exam questions and long answer responses and using transformer-based language models for automated grading. We prioritize the privacy and confidentiality of the individuals whose responses are being used for training and evaluation purposes. All data used in this research are anonymized and securely stored. Personal identifying information is removed to ensure the privacy of the participants. Moreover, automated grading systems are designed to assist human evaluators, not replace them entirely. We emphasize responsible use and the complementary role of automated grading alongside human assessment. By adhering to these ethical principles, we aim to ensure the protection of participant privacy and the responsible integration of automated grading systems into educational settings.

==> sections/method_and_dataset.tex <==
\input{figures/rubrichem_example}
In this section, we first present the problem formulation of the \model task followed by details on the \dataset dataset. 
The workflow of the \model system is also illustrated with details in Figure \ref{fig:flow}.

\subsection{\longmodel (\modelns)}

Let an inference model $M: (P, H) \rightarrow {L}$ be give, which takes a premise $P$ and a hypothesis $H$ as inputs and predicts a label $L \in \{True, False\}$ indicating whether $P$ \textit{entails} $H$.
To formulate grading as an inference problem, a student response $R$ and a rubric item $I$ can be treated as the premise and hypothesis respectively such that $(R, I) \xrightarrow{M} L$.

Our \model approach implements the aforementioned formulation by training a  language model to predict the entailment of a rubric item from a student response.
The predictions can effectively pinpoint the correctly or incorrectly addressed rubric items in the student response, consequently providing automated feedback.


\subsection{\dataset Dataset}
To investigate the potential benefits of incorporating rubric information in the \model model, we developed \dataset dataset.
This dataset not only serves as a valuable resource for researchers working on LAG, but also paves the way for the creation of more reliable and interpretable grading systems that can provide meaningful feedback to students.

\dataset features 4 exam questions, 27 rubric items, and 1264 graded student responses from a college-level chemistry course. Multiple teaching assistants graded the student responses against individual rubric items by assigning a TRUE or FALSE label. There are a total of 4880 TRUE labels and 3512 FALSE labels.
Each rubric item holds a designated point value, and the final score for a response is determined by aggregating the scores of rubric items that are correctly answered.
% To ensure a standardized scale, the scores are subsequently normalized to a range of 0 to 8.

==> sections/story.tex <==
In this research paper, we delve into the challenge of Long Answer Grading (LAG), a relatively unexplored area in the field of educational Natural Language Processing (NLP). Traditionally, the lack of a comprehensive dataset for long answer responses has limited the scope of study in this area. To overcome this hurdle and enable a thorough investigation, we have curated a specialized dataset, ChemLag, specifically designed for the LAG problem.

The primary focus of our study is the innovative framing of LAG as a rubric entailment problem. The conventional Automated Short Answer Grading (ASAG) employs a 5-way classification formulation, categorizing answers as "correct, partially correct, contradictory, irrelevant or not in the domain". However, we argue that this classification system is not entirely suitable for grading long answers, as such responses can simultaneously exhibit characteristics of multiple categories. Instead, a more nuanced and detailed evaluation approach that considers the multifaceted nature of long answers is required.

As an alternative, we propose a rubric-based approach, where each rubric item represents a specific criterion that the student's answer should meet. Then, we use natural language inference models to determine if each rubric item is entailed in the student's response. This provides a more comprehensive, point-by-point assessment, offering a more transparent and consistent grading standard.

Our research involves the utilization of fine-tuned encoder models like BERT, as well as the exploration of the performance of Generative Pre-trained Transformer (GPT) models. We present our findings on the effectiveness of these models in the context of our rubric-based LAG approach.

However, our research also underscores that the task of Long Answer Grading (LAG) is considerably more challenging compared to Automated Short Answer Grading (ASAG). This is evidenced by the comparative performance of the GPT model on ASAG's SciEntsBank, which achieved an F1 score of 0.74 without the use of rubrics, and our ChemLag dataset, which achieved a lower score of 0.69, despite the use of rubrics. 

It's noteworthy that the use of rubrics generally enhances model performance, as they provide a detailed, point-by-point assessment framework. Thus, the fact that our model achieved a lower score on ChemLag, even with the advantage of rubrics, emphasizes the increased complexity and challenge posed by LAG. The actual difference in difficulty between ASAG and LAG may be even more significant than the 5-point difference in F1 scores suggests.

Through this work, we aim to contribute to the advancement of educational NLP by providing a more nuanced and effective approach for grading long answers, and by introducing a new dataset that can facilitate further research in this area.


Next section should be related work.
Talk about 5-way classes of scientsbank.

Next section should be dataset
two paras are there..
most important info is avg. word size.
next most important info is rubrics are there.

Next section should be LAG formulation.
talk about both rubric and score based formulation (without referring to asag)

Next section should be results
- model training
- baselines
- score vs rubric formulation (no mention of asag)
- end with GPT

Conclusion


==> tables/baselines_table_compressed.tex <==
% \begin{table}[h]
% \centering
% \normalsize
% \begin{tabular}{lllll}
%   \hline
%   \textbf{Model} & \textbf{Accuracy} & \textbf{F1} \\
%   \hline
%   BERT-base & 0.821 & 0.786 \\
%   BERT-large & 0.834 & 0.800 \\
%   RoBERTa-base & 0.834 & 0.799 \\ 
%   RoBERTa-large & 0.849 & 0.822 \\
%   BART-base & 0.827 & 0.790 \\
%   BART-large & 0.845 & 0.815 \\
%   \hline
% \end{tabular}
% % \captionsetup{width=\textwidth}
% \caption{Performance of base and large discriminative language models. The large models outperform the base models by a large enough margin, showing that the level of the difficulty of the task requires larger models on \datasetns.}
% \label{tab:baselines} 
% \end{table}

==> tables/comparison_table_compressed.tex <==
% \begin{table}[t]
% \begin{tabular}{llll}
% \hline
% \textbf{Model}     & \textbf{\modelns} & \textbf{Accuracy} & \textbf{F1} \\ \hline
% BERT-base          & \xmark          & 0.424  & 0.361           \\
%                    & \cmark          & \textbf{0.490}  & \textbf{0.434}           \\ \hline
% BERT-large         & \xmark           & 0.422  & 0.380           \\
%                    & \cmark          & \textbf{0.477}  & \textbf{0.439}           \\ \hline
% RoBERTa-base       & \xmark           & 0.435  & 0.404           \\
%                    & \cmark           & \textbf{0.515}  & \textbf{0.497}           \\ \hline
% RoBERTa-large      & \xmark            & 0.449  & 0.403           \\
%                    & \cmark         & \textbf{0.502}  & \textbf{0.478}           \\ \hline
% BART-base          & \xmark            & 0.438  & 0.380           \\
%                    & \cmark          & \textbf{0.468} & \textbf{0.430}           \\ \hline
% BART-large         & \xmark          & 0.461  & 0.428           \\
%                    & \cmark          & \textbf{0.504}  & \textbf{0.489}          \\ \hline
% \end{tabular}
% \caption{Comparisons of \model and the traditional ASAG approach on \dataset dataset. We observe an improvement of performance in the accuracy and F1 score from applying \modelns. Breaking down grading into smaller rubric items helps models focus on smaller parts of the task instead of doing the entire task altogether. The improvement is evident across all models regardless of their size.}
% \label{tab:comparisons}
% \end{table}

==> tables/comparisons_table.tex <==
% \begin{table*}
% \centering
% \normalsize
% \begin{tabular}{llllllll}
% \hline
% \textbf{Model} & \textbf{Method} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{MSE} & \textbf{MAE} \\
% \hline
% BERT-base-uncased & ASAG & 0.424 & 0.359 & 0.380 & 0.361 & 2.885 & 1.096 \\
% & \model & 0.490 & 0.432 & 0.451 & 0.434 & 2.461 & 0.932 \\ 
% \hline
% BERT-large-uncased & ASAG & 0.422 & 0.397 & 0.400 & 0.380 & 2.929 & 1.109 \\
% & \model & 0.477 & 0.445 & 0.455 & 0.439 & 2.195 & 0.908\\
% \hline
% BERT-large-mnli & ASAG & 0.417 & 0.370 & 0.373 & 0.353 & 2.909 & 1.132\\
% & \model & 0.499 & 0.489 & 0.472 & 0.475 & 2.144 & 0.883 \\
% \hline
% RoBERTa-base & ASAG & 0.435 & 0.420 & 0.413 & 0.404 & 2.625 & 1.028 \\
% & RASAG & 0.515 & 0.500 & 0.514 & 0.497 & 2.508 & 0.906 \\ 
% \hline
% RoBERTa-large & ASAG & 0.449 & 0.414 & 0.414 & 0.403 & 2.458 & 0.997\\
% & \model & 0.502 & 0.479 & 0.494 & 0.478 & 2.189 & 0.867\\
% \hline
% RoBERTa-large-mnli & ASAG & 0.424 & 0.391 & 0.394 & 0.378 & 2.929 & 1.128 \\
% & \model & 0.561 & 0.552 & 0.537 & 0.536 & 2.013 & 0.772\\
% \hline
% BART-base & ASAG & 0.438 & 0.373 & 0.407 & 0.380 & 2.917 & 1.096 \\
% & \model & 0.4677 & 0.440 & 0.445 & 0.430 & 2.528 & 0.963 \\
% \hline
% BART-large & ASAG & 0.461 & 0.430 & 0.458 & 0.428 & 2.874 & 1.060\\
% & \model & 0.504 & 0.497 & 0.502 & 0.489 & 2.595 & 0.903 \\
% \hline
% BART-large-mnli & ASAG & 0.391 & 0.366 & 0.371 & 0.357 & 3.150 & 1.194\\
% & \model & 0.521 & 0.538 & 0.501 & 0.506 & 1.903 & 0.806\\
% \hline
% % GPT3.5 & ASAG & 0.208 & 0.145 & 0.186 & 0.137 & 9.633 & 2.483 \\
% % & \model & 0.260 & 0.176 & 0.274 & 0.164 & 8.077 & 2.115\\
% % \hline
% % GPT4 & ASAG & 0.175 & 0.218 & 0.147 & 0.129 & 8.460 & 2.365 \\
% % & \model & 0.280 & 0.296 & 0.289 & 0.221 & 6.072 & 1.768\\
% % \hline
% \end{tabular}
% \caption{\label{tab:results1} Comparisons of \model and the traditional ASAG approach. We observe significant improvement of performance across all the metrics from applying \modelns. The improvement can be benefited by all models regardless of their number of parameters. Breaking down grading into smaller rubric items is helps models focus on smaller parts of the task instead of doing the entire task altogether.}
% \end{table*}
